Joint Reconstruction and Parcellation of Cortical Surfaces

The reconstruction of cerebral cortex surfaces from brain MRI scans is instrumental for the analysis of brain morphology and the detection of cortical thinning in neurodegenerative diseases like Alzheimer's disease (AD). Moreover, for a fine-grained analysis of atrophy patterns, the parcellation of the cortical surfaces into individual brain regions is required. For the former task, powerful deep learning approaches, which provide highly accurate brain surfaces of tissue boundaries from input MRI scans in seconds, have recently been proposed. However, these methods do not come with the ability to provide a parcellation of the reconstructed surfaces. Instead, separate brain-parcellation methods have been developed, which typically consider the cortical surfaces as given, often computed beforehand with FreeSurfer. In this work, we propose two options, one based on a graph classification branch and another based on a novel generic 3D reconstruction loss, to augment template-deformation algorithms such that the surface meshes directly come with an atlas-based brain parcellation. By combining both options with two of the latest cortical surface reconstruction algorithms, we attain highly accurate parcellations with a Dice score of 90.2 (graph classification branch) and 90.4 (novel reconstruction loss) together with state-of-the-art surfaces.

==> tables/Mindboggle.tex <==
\begin{table}
    \footnotesize
    %\setlength{\tabcolsep}{1pt} % Reduce white-space between columns, SHOULD BE SET AFTER TABLE IS FINISHED
    
    %0.453 \interval{0.072} 
    \begin{adjustbox}{width=1\textwidth}
    
        \begin{tabular}{lcccccc}
            \toprule
            & \multicolumn{3}{c}{White surface} 
    & \multicolumn{3}{c}{Pial surface}
    \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-7}
    Method & Dice & AD & HD  & Dice & AD & HD\\\midrule
            \midrule
            FreeSurfer~\cite{freesurferv7.2} & 0.871 \interval{0.088}& xx &xx & & & \\
            SegRecon~\cite{gopinath2021}* & 0.887 \interval{0.018} & xx &xx & & & \\
            V2C + temp & & & & & & \\
            V2C+ class & & & & & & \\
            CorticalFlow + temp & & & & & &  \\
            CorticalFlow + class & & & & & &  \\

            \bottomrule
        \end{tabular}
    \end{adjustbox}
    \caption{Comparison of parcellation quality of the extended Vox2Cortex and CorticalFlow with FreeSurfer, FastSurfer and SegRecon on the Mindboggle dataset. * values taken from ~\cite{gopinath2021}}
    \label{tab:parcellation}
\end{table}

==> tables/comparison.tex <==
\begin{table*}
\footnotesize
\setlength{\tabcolsep}{1pt} % Reduce white-space between columns, SHOULD BE SET AFTER TABLE IS FINISHED

%0.453 \interval{0.072} 
\begin{adjustbox}{width=1\textwidth}

\begin{tabular}{llcccccccc}
    \toprule
    & & \multicolumn{2}{c}{Left WM} 
    & \multicolumn{2}{c}{Right WM}
    & \multicolumn{2}{c}{Left Pial}
    & \multicolumn{2}{c}{Right Pial}

    \\
    \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
    Data & Method & AD & HD  & AD & HD  & AD & HD & AD & HD\\\midrule
    
%     \multirow{3}{*}{\makecell{ADNI\\orig}} & \gls{exprecs} & 0.359 \interval{0.116} & 0.795 \interval{0.332} & 0.356 \interval{0.107} & 0.777 \interval{0.317} & 0.314 \interval{0.084} & 0.711 \interval{0.236} & 0.311 \interval{0.079} & 0.699 \interval{0.225} 
%     %& 0.335 \interval{0.100} & 0.745 \interval{0.285} \\ 
%   \\
%     \addlinespace[0.3em]
%     & DeepCSR~\cite{santacruz2021}*  & 0.267 \interval{0.216} & 0.562 \interval{0.725} & 0.260 \interval{0.162} &  0.542 \interval{0.523}& 0.298 \interval{0.184}  & 0.654 \interval{0.596} & 0.294 \interval{0.155}& 0.651 \interval{0.530} \\
%     \addlinespace[0.3em]
%     & nnUNet &1.146 \interval{0.203} & 1.674 \interval{1.481}  & 1.162 \interval{0.317}  & 1.865 \interval{2.808}  & 1.120 \interval{0.169}  & 2.391 \interval{1.267} & 1.191 \interval{0.129}& 2.418 \interval{0.951} \\
%     \addlinespace[0.3em]
    
    %\midrule
    \multirow{5}{*}{\makecell{ADNI}} & ours & & & & & & & & 
    \\ 
    \addlinespace[0.3em]
    
    & Vox2Cortex(53) & \textbf{0.345} \interval{0.056} & \textbf{0.720} \interval{0.125} & \textbf{0.347} \interval{0.046} & \textbf{0.720} \interval{0.087} & \textbf{0.327} \interval{0.031} & \textbf{0.755} \interval{0.102} & \textbf{0.318} \interval{0.029} & \textbf{0.781} \interval{0.102} \\
    & Vox2Cortex(72) & \textbf{0.318} \interval{0.0489} & \textbf{0.729} \interval{0.135} & \textbf{0.320} \interval{0.040} & 0.725 \interval{0.110} & \textbf{0.330} \interval{0.038} & \textbf{0.814} \interval{0.097} & \textbf{0.330} \interval{0.033} & \textbf{0.825} \interval{0.096}\\ 
    %& 0.334 \interval{0.044} & 0.744 \interval{0.108} \\ 
   \\
    \addlinespace[0.3em]
    & DeepCSR(53)~\cite{santacruz2021}  & 0.422 \interval{0.058} &0.852 \interval{0.134} & 0.420 \interval{0.058}  & 0.880 \interval{0.156} & 0.454 \interval{0.059} & 0.927 \interval{0.243} & 0.422 \interval{0.053}& 0.890 \interval{0.197}\\
    \addlinespace[0.3em]
    & FastSurfer(72)~\cite{henschel2020} & 0.150 \interval{0.061}& 0.339 \interval{0.162} & 0.151 \interval{0.063}&  0.345 \interval{0.183}  & 0.190 \interval{0.044}  & 0.371 \interval{0.119}  & 0.191 \interval{0.045}  & 0.368 \interval{0.118}  \\
    \addlinespace[0.3em]
    & Cortical Flow & &  & &    &   &   &   &   \\
    \addlinespace[0.3em]
    
    \midrule
    \multirow{5}{*}{OASIS} & ours & & & & & & & & 
    \\ 
    \addlinespace[0.3em]
     & Vox2Cortex(53) & \textbf{0.315} \interval{0.039} & \textbf{0.680} \interval{0.137} & \textbf{0.318} \interval{0.048} & 0.682 \interval{0.151} & \textbf{0.362} \interval{0.036} & \textbf{0.894} \interval{0.141} & \textbf{0.373} \interval{0.041} & \textbf{0.916} \interval{0.137}\\ 
     & Vox2Cortex(72) & \textbf{0.294} \interval{0.044} & \textbf{0.633} \interval{0.123} & \textbf{0.296} \interval{0.055} & 0.639 \interval{0.153} & \textbf{0.347} \interval{0.035} & \textbf{0.866} \interval{0.131} & \textbf{0.352} \interval{0.041} & \textbf{0.873} \interval{0.138}\\ 
 
    \addlinespace[0.3em]
    & DeepCSR(53)~\cite{santacruz2021}  & 0.360 \interval{0.042}&0.731 \interval{0.104} & 0.335 \interval{0.050}& \textbf{0.670} \interval{0.195}  &  0.458 \interval{0.056} & 1.044 \interval{0.290}  & 0.442 \interval{0.058}  & 1.037 \interval{0.294}  \\
    & FastSurfer(72)~\cite{henschel2020} & 0.135 \interval{0.044}& 0.318 \interval{0.136} & 0.141 \interval{0.071}& 0.344 \interval{0.207}   & 0.234 \interval{0.051}& 0.532 \interval{0.131}   & 0.247 \interval{0.078}  & 0.582 \interval{0.227}  \\
    \addlinespace[0.3em]
    & Cortical Flow & &  & &    &   &   &   &   \\
    \bottomrule
\end{tabular}
\end{adjustbox}
\caption{Comparison of mesh quality of our extended Vox2Cortex with Vox2Cortex, DeepCSR, FastSurfer and CorticalFlow on the ADNI and OASIS datasets for the four surfaces. All values are in mm.}
\label{tab:comparison}
\end{table*}

% \begin{tabular}{llcccccccccl}
%     \toprule
%     & & \multicolumn{2}{c}{Left WM Surface} 
%     & \multicolumn{2}{c}{Right WM Surface}
%     & \multicolumn{2}{c}{Left Pial Surface}
%     & \multicolumn{2}{c}{Right Pial Surface}
%     & \multicolumn{2}{c}{All Surfaces}
%     \\
%     \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12}
%     Data & Method & AD  & HD & AD & HD  & AD & HD & AD & HD & AD & HD \\\midrule
    
%     \multirow{3}{*}{\makecell{ADNI\\orig}} & \gls{exprecs} & &  &  &  &  &  & &  &  & \\
%     \addlinespace[0.5em]
%     & DeepCSR~\cite{santacruz2021}*  & 0.267 \interval{0.216} & 0.562 \interval{0.725} & 0.260 \interval{0.162} &  0.542 \interval{0.523}& 0.298 \interval{0.184}  & 0.654 \interval{0.596} & 0.294 \interval{0.155}& 0.651 \interval{0.530} & 0.280 \interval{0.179} & 0.602 \interval{0.594} \\
%     \addlinespace[0.5em]
%     & nnUNet &0.735 \interval{1.235} & 1.312 \interval{3.856}  & 0.777 \interval{1.584}  & 1.490 \interval{4.296}  & 0.904 \interval{1.223}  & 1.984 \interval{4.057} & 0.950 \interval{1.481}& 2.231 \interval{4.492} & 0.842 \interval{1.223} & 1.754 \interval{4.057} \\
%     \addlinespace[0.5em]
    
%     \midrule
%     \multirow{2}{*}{OASIS} & \gls{exprecs} & 0.315 \interval{0.039} & 0.680 \interval{0.137} & 0.318 \interval{0.048} & 0.682 \interval{0.151} & 0.362 \interval{0.036} & 0.894 \interval{0.141} & 0.373 \interval{0.041} & 0.916 \interval{0.137} & 0.342 \interval{0.049} & 0.793 \interval{0.181} \\ 
 
%     \addlinespace[0.5em]
%     & DeepCSR  & &  &  &  &  &  & &  &  & \\
%     \bottomrule
% \end{tabular}
